Raw-to-End Name Entity Recognition in Social Media

Taking word sequences as the input, typical named entity recognition (NER) models neglect errors from pre-processing (e.g., tokenization). However, these errors can influence the model performance greatly, especially for noisy texts like tweets. Here, we introduce Neural-Char-CRF, a raw-to-end framework that is more robust to pre-processing errors. It takes raw character sequences as inputs and makes end-to-end predictions. Word embedding and contextualized representation models are further tailored to capture textual signals for each character instead of each word. Our model neither requires the conversion from character sequences to word sequences, nor assumes tokenizer can correctly detect all word boundaries. Moreover, we observe our model performance remains unchanged after replacing tokenization with string matching, which demonstrates its potential to be tokenization-free. Extensive experimental results on two public datasets demonstrate the superiority of our proposed method over the state of the art. The implementations and datasets are made available at: https://github.com/LiyuanLucasLiu/Raw-to-End.

==> 8benchmark.tex <==
% !TEX encoding = UTF-8
% !TEX Root = 0_main.tex


\section{Experiment}
\label{sec:benchmark}

% \heng{Also I guess it's probably too late, it would have been interesting to try your model on clinical notes NER:
% https://clinical-nlp.github.io/2019/resources.html}

In this section, we conduct extensive experiments to verify the effectiveness of the 

formulate the s to raw-to-end named entity recognition (NER) task, then establish its benchmarks on Twitter. 
In detail, we convert two existing Twitter NER benchmark datasets from word-level labels to character-level labels and create a new dataset by directly annotating at the character level.
On these three datasets, we evaluate state-of-the-art NER models paired with popular pre-processing methods and discuss the key challenges.

% \subsection{Problem Formulation}

% We formulate the raw-to-end NER task as a character-level sequence labeling problem.
% The input is a character sequence $X=\{x_1, x_2, \ldots, x_T\}$, where $x_i$ $(1 \le i \le T)$ is the $i$-th character and $T$ is the length.
% Following popular labeling schemes like \texttt{IOB} and \texttt{IOBES}~\cite{ratinov2009design}, we assign a label for each character.
% We refer the label for $x_i$ as $\y_i$.
% The goal of the raw-to-end NER is to predict the label sequence $\Y = \{\y_1, \y_2, \ldots \y_T\}$.

\input{tbl_stat.tex}

\subsection{Benchmark Datasets}

    We prepared three benchmark datasets (i.e., TNT, BTC, and TWIN) for raw-to-end NER on Twitter -- TNT and BTC are recovered from word level annotations, TWIN is directly annotated at the character level. Their statistics can be found in Table~\ref{tab:stat}.

    \subsubsection{Label Conversion from Word Level}
    
        Typical NER benchmark datasets are annotated on pre-processed word sequence.
        Such pre-processing includes but is not limited to adding/removing whitespaces by tokenization, spelling changes due to normalization, and even language changes using translation.
        Consequently, converting these labels to  character level requires the original raw texts.
        We find that two Twitter NER datasets, as follows, meet this requirement:
        (1) \textbf{TNT}~\cite{lu2018visual} contains tweets from May 2016, January 2017 and June 2017, retrieved by using sports and social event related keywords.
        and (2) \textbf{BTC}~\cite{derczynski2016broad} contains tweets from various periods and regions, related to diverse topics. 
        TNT is annotated with four types (\texttt{PER}, \texttt{LOC}, \texttt{ORG} and \texttt{MISC}), while BTC only has the first three types.
        We adopt their recommended data split for training, development and testing sets. 

        We have designed several rules (detailed in Appendix~\ref{app:untokenize}) to map the pre-processed words back to the original raw texts and export character-level annotations. 
        
\input{tbl_all_f1.tex}
    \subsubsection{New Dataset Construction}
    
        We have paid tremendous effort to convert word-level annotations to character-level annotations, however, this is not ideal for raw-to-end benchmarks.
        For example, the annotators can never mark the two entities ``Lakers'' and ``Raptors'' correctly, if the presented word sequence only has ``Lakers-Raptors''.
% move to 1 para earlier? 
        Therefore, some desired character-level annotations can be missing in the word-level annotations, because of the non-perfect pre-processing during the dataset construction stage.
        
        We construct a new dataset by annotating at the character level directly: we collect 6,500 tweets from January 2015 to December 2015, filter out non-English tweets, then recruit multiple annotators to manually label the entities of four types (\texttt{PER}, \texttt{LOC}, \texttt{ORG} and \texttt{MISC}). 
        For quality control purpose, each tweet is annotated by at least two annotators. 
        After initial annotations, we further conduct an additional round of calibrations.
        We refer our new dataset as \textbf{TWIN}. 

    \subsection{Benchmark Evaluation}
    
        Based on above three datasets, we establish the raw-to-end NER benchmarks on Twitter.
        In our practice, we evaluate four state-of-the-art (Twitter) NER models with three popular pre-processing methods, which form \emph{twelve combinations}.
        During the model training and evaluation, we tokenize the input characters and feed them into the NER model.
        Training details are introduced in Appendix~\ref{app:training}, and implementation details, including how to tweak training labels after the tokenizers are applied, can be found in Appendix~\ref{app:preprocess}.
% consider active voice?

% we considered -> we evaluated?
        The four NER models we considered are:
        \begin{enumerate}[nosep,leftmargin=*]
            \item \textbf{TwitterNER}~\cite{mishra2016_wnut_ner} is specifically designed for tweets. It relies on not only handcrafted features, but also domain-specific resources.
            \item \textbf{LSTM-CNNs-CRF}~\cite{ma2016end} does not rely on feature engineering and constructs the sequence labeling in an end-to-end manner. 
            \item \textbf{LM-LSTM-CRF}~\cite{liu2018empower} is a sequence labeling model, which integrates language models without pre-training and uses them to construct representations.
% without pre-training? model/representation
            \item \textbf{Flair}~\cite{akbik2018contextual} leverages language models to construct contextualized word representations and achieves the state-of-the-art performance on English NER for news corpus. 
        \end{enumerate}
        For pre-processing, we considered three tokenizers:
        \begin{enumerate}[leftmargin=*,nosep]
            \item \textbf{spaCy}~\cite{spacy2} employs the NLP package spaCy for tokenization, which features efficiency and effectiveness\footnote{SpaCy 2.0.18 is used.}. 
            \item \textbf{Stanford CoreNLP}~\cite{manning-EtAl:2014:P14-5} leverages the widely used Stanford CoreNLP~\cite{manning-EtAl:2014:P14-5} as tokenizer\footnote{The version 3.9.2 release is used.}.
            \item \textbf{NLTK}~\cite{bird2008multidisciplinary} is a leading platform for building NLP pipelines and we only used its tokenization module here\footnote{The version 3.4 release is used.}.
        \end{enumerate}

\input{tbl_two_step.tex}

    \subsection{Benchmark Results}
    
        We present the evaluation results in Table~\ref{tab:all}.
        One can easily observe that the tokenizer plays an crucial role on the performance, especially on the BTC and TWIN datasets.
        For example, switching the tokenizer from NLTK to spaCy or Stanford CoreNLP leads to a drop of more than 20 \fl points. 
        
        % We further investigated whether using the gold-tokenized training data can benefit its performance in evaluation with the best performing NLTK tokenizer.
        % The results summarized in Table~\ref{tab:two_step} show \fl performance drops in most cases.
        % Therefore, the NER performance is limited by the tokenizer.
        
        We further conduct experiments to verify our intuition of fusing pre-processing with sequence labeling. 
        Specifically, we construct models with gold-tokenized training data and evaluate their performance with NLTK, which achieves the best performance among all three tokenizers. 
        The results summarized in Table~\ref{tab:two_step} show that, after replacing NLTK-tokenized training data with gold-tokenized training data, \fl drops in most cases.
        It verifies our intuition to build the raw-to-end benchmark, which allows us to jointly optimize and evaluate NER models. 
       % and the idea of building?
%         ind the results 
% in favor of 
%  joint optimization.
 
        

==> tbl_all.tex <==
% !TEX encoding = UTF-8
% !TEX Root = 0_main.tex

\begin{table*}[t]
\begin{center}
\caption{Performance Comparison. \xiang{make the caption more self-contained for interpreting the results? use scalebox to shrink down size.}}
\label{tab:all}
\begin{tabularx}{\linewidth}{c c *{9}{Y}}
\toprule
\multirow{2}{*}{Tokenizer} & \multirow{2}{*}{Methods} & \multicolumn{3}{c}{TWIN} & \multicolumn{3}{c}{TNT} & \multicolumn{3}{c}{BTC} \\\cmidrule{3-11}
& & Pre & Rec & \fl & Pre & Rec & \fl & Pre & Rec & \fl \\\midrule

% \multicolumn{2}{c}{\our} & \textbf{86.69}	& \textbf{85.61} & \textbf{86.15} \\\midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} NLTK  \end{tabular}}

  &   TwitterNER   & 71.77 & 60.05 & 65.39 & 76.84 & 72.07 & 73.41 & 71.12 & 58.84 & 64.40\\
  &   LSTM-CNN-CRF & 71.59 & 65.82 & 68.59 & 83.05 & 77.63 & 80.25 & 75.20 & 59.57 & 66.48\\
  &   LM-LSTM-CRF  & 70.43 & 64.67 & 67.43 & 81.66 & 80.05 & 80.85 & 74.80 & 61.88 & 67.73\\
  &   Flair        & 73.65 & 66.97 & 69.91 & 85.08 & 81.51 & 83.26 & 76.49 & 61.74 & 68.33 \\\midrule\midrule
  
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}spaCy\end{tabular}}

  &   TwitterNER   & 60.62 & 33.74 & 43.35 & 80.96 & 62.27 & 70.40 & 67.73 & 25.65 & 37.21\\
  &   LSTM-CNN-CRF & 15.62 & 13.46 & 14.46 & 73.54 & 69.87 & 71.66 & 33.28 & 25.76 & 29.04 \\
  &   LM-LSTM-CRF  & 21.58 & 19.79 & 20.65 & 73.03 & 71.50 & 72.25 & 34.11 & 28.70 & 31.17 \\
  &   Flair        & 52.92 & 20.83 & 29.89 & 74.39 & 72.80 & 73.49 & 37.31 & 29.90 & 33.20 \\\midrule\midrule

\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Stanford \\CoreNLP \end{tabular}}

  &   TwitterNER   & 47.72 & 29.47 & 36.43 & 79.86 & 62.59 & 70.18 & 69.26 & 26.19 & 38.01 \\
  &   LSTM-CNN-CRF & 21.97 & 20.02 & 20.95 & 66.25 & 62.31 & 64.22 & 35.59 & 25.49 & 29.71 \\
  &   LM-LSTM-CRF  & 15.51 & 13.92 & 14.68 & 63.63 & 62.67 & 63.14 & 32.36 & 26.23 & 28.97 \\
  &   Flair        & 48.42 & 15.88 & 23.92 & 66.46 & 64.73 & 65.58 & 36.84 & 28.90 & 32.39 \\
\bottomrule
\end{tabularx}
\end{center}
\vspace{-0.3cm}
\end{table*}


==> tbl_btc.tex <==
% !TEX encoding = UTF-8
% !TEX Root = 0_main.tex

\begin{table}[t]
\begin{center}
\caption{Performance Comparison on the BTC Dataset.}
\label{tab:btc}
\begin{tabularx}{\columnwidth}{c c *{3}{Y}}
\toprule
\multirow{2}{*}{Tokenizer} & \multirow{2}{*}{Methods} & \multicolumn{3}{c}{BTC} \\\cmidrule{3-5}
& & Pre & Rec & \fl \\\midrule
% \multicolumn{2}{c}{\our} & \textbf{77.57}	& \textbf{71.39} & \textbf{74.35} \\\midrule

\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}} \textit{Expert-} \\ \textit{tokenized} \end{tabular}}

  &   StanfordNER & 74.61 & 54.93 & 63.27 \\
  &   TwitterNER & 70.89 & 61.18 & 65.67 \\
  &   LM-LSTM-CRF & 73.30 & 65.59 & 69.29 \\\midrule\midrule
  
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}spaCy\end{tabular}}

  &   StanfordNER & 30.95 & 20.68 & 24.79 \\
  &   TwitterNER & 67.73 & 25.65 & 37.21 \\
  &   LM-LSTM-CRF & 34.11 & 28.70 & 31.17 \\\midrule

\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Stanford \\CoreNLP \end{tabular}}

  &   StanfordNER & 31.84 & 21.42 & 25.61 \\
  &   TwitterNER & 69.26 & 26.19 & 38.01 \\
  &   LM-LSTM-CRF & 32.36 & 26.23 & 28.97 \\\midrule\midrule

\diagbox{}{} & \our & \textbf{79.52}	& \textbf{70.93} & \textbf{74.98} \\
\bottomrule
\end{tabularx}
\end{center}
\vspace{-0.3cm}
\end{table}



\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{error_prop.pdf}
  \caption{Stacked bar chart for tokenization error analysis. After switching from gold-standard tokenization results (\textit{expert-tokenized}) to the ones got from spaCy / Stanford CoreNLP, the appeared error instantly deteriorate the model performance. At the same time, our raw-to-end model neither rely on pre-processing nor suffer from such errors. }
%   \Description{Case study for the error propagation.}
  \label{fig:prop}
  \vspace{-0.3cm}
\end{figure}

==> tbl_tnt.tex <==
% !TEX encoding = UTF-8
% !TEX Root = 0_main.tex

\begin{table}[t]
\begin{center}
\caption{Performance Comparison on the TNT Dataset.}
\label{tab:tnt}
\begin{tabularx}{\columnwidth}{c c *{3}{Y}}
\toprule
\multirow{2}{*}{Tokenizer} & \multirow{2}{*}{Methods} & \multicolumn{3}{c}{TNT} \\\cmidrule{3-5}
& & Pre & Rec & \fl \\\midrule

% \multicolumn{2}{c}{\our} & \textbf{86.69}	& \textbf{85.61} & \textbf{86.15} \\\midrule
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}} \textit{Expert-} \\ \textit{tokenized}  \end{tabular}}

  &   VAG-BLSTM-CRF & 81.62 & 79.90 & 80.75 \\
  &   StanfordNER & 82.08 & 66.35 & 73.38 \\
  &   TwitterNER & 76.70 & 69.83 & 73.24  \\
  &   LM-LSTM-CRF & 82.17 & 81.71 & 81.94 \\\midrule\midrule
  
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}spaCy\end{tabular}}

  &   StanfordNER & 73.10 & 58.51 & 65.00 \\
  &   TwitterNER & 80.96 & 62.27 & 70.40 \\
  &   LM-LSTM-CRF & 73.03 & 71.50 & 72.25 \\\midrule

\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Stanford \\CoreNLP \end{tabular}}

  &   StanfordNER & 67.10 & 53.44 & 59.50 \\
  &   TwitterNER & 79.86 & 62.59 & 70.18 \\
  &   LM-LSTM-CRF & 63.63 & 62.67 & 63.14 \\\midrule\midrule
  
\diagbox{}{} & \our & \textbf{87.41}	& \textbf{86.51} & \textbf{86.96} \\
\bottomrule
\end{tabularx}
\end{center}
\vspace{-0.3cm}
\end{table}


==> tbl_tok.tex <==
% !TEX encoding = UTF-8
% !TEX Root = 0_main.tex
% \parbox{\linewidth}{

\begin{table}[t]
\begin{center}
\caption{Dataset Statistics of TNT, BTC and TWIN.}
\label{tab:stat}
% \scalebox{0.7}{
\begin{tabularx}{1.4\columnwidth}{r *{3}{Y}}
\toprule
            &   TNT &   BTC &   TWIN \\\midrule
# Entities  &   5332

\bottomrule
\end{tabularx}
% }
\end{center}
\vspace{-0.3cm}
\end{table}

